Layered State Discovery for Incremental Autonomous Exploration

We study the autonomous exploration (AX) problem proposed by Lim & Auer (2012). In this setting, the objective is to discover a set of $\epsilon$-optimal policies reaching a set $\mathcal{S}_L^{\rightarrow}$ of incrementally $L$-controllable states. We introduce a novel layered decomposition of the set of incrementally $L$-controllable states that is based on the iterative application of a state-expansion operator. We leverage these results to design Layered Autonomous Exploration (LAE), a novel algorithm for AX that attains a sample complexity of $\tilde{\mathcal{O}}(LS^{\rightarrow}_{L(1+\epsilon)}\Gamma_{L(1+\epsilon)} A \ln^{12}(S^{\rightarrow}_{L(1+\epsilon)})/\epsilon^2)$, where $S^{\rightarrow}_{L(1+\epsilon)}$ is the number of states that are incrementally $L(1+\epsilon)$-controllable, $A$ is the number of actions, and $\Gamma_{L(1+\epsilon)}$ is the branching factor of the transitions over such states. LAE improves over the algorithm of Tarbouriech et al. (2020a) by a factor of $L^2$ and it is the first algorithm for AX that works in a countably-infinite state space. Moreover, we show that, under a certain identifiability assumption, LAE achieves minimax-optimal sample complexity of $\tilde{\mathcal{O}}(LS^{\rightarrow}_{L}A\ln^{12}(S^{\rightarrow}_{L})/\epsilon^2)$, outperforming existing algorithms and matching for the first time the lower bound proved by Cai et al. (2022) up to logarithmic factors.

==> sections/pc.tex <==
\section{Policy Consolidation}
\label{sec:pc}
Algorithms introduced in previous sections discover a set $\calK$ such that $\acalS_L\subseteq\calK\subseteq\acalS_{L(1+\epsilon)}$ and a set of goal-conditioned policies satisfying $\AX_L$.
In this section, we introduce an algorithm that takes a set $\calK\subseteq\acalS_{L(1+\epsilon)}$ as input, and learns a set of goal-condition policies satisfying the $\AX^+$ condition.

Our algorithm has a similar structure as \valve: the whole learning procedure is divided into rounds.
In each round, we randomly select an ``unknown'' goal state from $\calL$ and compute a policy to reach it (\pref{line:}).
We then evaluate the performance of this policy by $\tilo{\frac{1}{\epsilon^2}}$ rollouts, and based on the evaluation result, the current round is classified into success, skip, or failure round similar to that in \pref{alg:LOGSSD}.
The crucial difference compared to \valve is the condition of success round (\pref{line:}), which has a form similar to $\AX^+$.
Thus, one can treat \pref{alg:PC} as an improved version of \valve.
The guaranetee of \pref{alg:PC} is as follows.

\begin{theorem}
    \label{thm:PC}
    Given a target state space $\tset\subseteq \acalS_{L(1+\epsilon)}$ for some $\epsilon\in(0, 1)$ and a set of initial policy $\Pi'=\{\pi'_g\}_{g\in\calK}$ such that $\norm{V^{\pi'_g}_g}_{\infty}\lesssim L$ for each $\pi'\in\Pi'$, with probability at least $1-\bigo{\delta}$, after collecting $\tilO{\frac{L\aS_{L(1+\epsilon)}A\ln^p(\aS_{L(1+\epsilon)})}{\epsilon^2}}$ (ignoring lower order terms) samples from the environment for some absolute constant $p\geq 1$, \pref{alg:PC} outputs a set of policies $\{\tilpi_g\}_{g\in\tset}$ such that $V^{\tilpi_g}_g(s_0)\leq \optV_{\tset,g}(s_0)(1+\epsilon)$ for all $g\in\tset$.
\end{theorem}

We develop an improved regret-based analysis to bound the total sample complexity of \pref{alg:PC}.
The key technical contribution here is that instead of bounding the total number of rounds as in \valve, we directly bound the total number of steps in all rounds, which takes varying length of trajectories in different rounds into consideration.
This enables \pref{alg:PC} to achieve a better sample complexity compared to \valve.
Note that \pref{alg:PC} can be combined with any set discovery algorithm (such as \ucbexplore and \disco) and give an algorithm satisfying $\AX^+$.
